Prompt-Guided Retrieval Augmentation for Non-Knowledge-Intensive Tasks

Retrieval-augmented methods have received increasing attention to support downstream tasks by leveraging useful information from external resources. Recent studies mainly focus on exploring retrieval to solve knowledge-intensive (KI) tasks. However, the potential of retrieval for most non-knowledge-intensive (NKI) tasks remains under-explored. There are two main challenges to leveraging retrieval-augmented methods for NKI tasks: 1) the demand for diverse relevance score functions and 2) the dilemma between training cost and task performance. To address these challenges, we propose a two-stage framework for NKI tasks, named PGRA. In the first stage, we adopt a task-agnostic retriever to build a shared static index and select candidate evidence efficiently. In the second stage, we design a prompt-guided reranker to rerank the nearest evidence according to task-specific relevance for the reader. Experimental results show that PGRA outperforms other state-of-the-art retrieval-augmented methods. Our analyses further investigate the influence factors to model performance and demonstrate the generality of PGRA. Codes are available at https://github.com/THUNLP-MT/PGRA.

==> Intro_V0.tex <==
Retrieval-augmented methods aim to find relevant evidence from knowledge resources for better handling downstream tasks. As a complementary method to the existing pre-trained models~\cite{devlin-etal-2019-bert,brown2020language}, such semi-parameter methods have been widely used for language modeling~\cite{khandelwal20generalization, pmlr-v119-guu20a, pmlr-v162-borgeaud22a}, machine translation~\cite{zhang-etal-2018-guiding,khandelwal2021nearest}, and question answering~\cite{lee-etal-2019-latent,karpukhin-etal-2020-dense,NEURIPS2020_6b493230,izacard-grave-2021-leveraging,izacard2022few}. 

% %These tasks, especially Knowledge Intensive tasks (KI;~\citealp{petroni-etal-2021-kilt}) which requires to access a large body of external information, can obviously benefit through nearest retrieved passages from a large knowledgeable corpus like Wikipedia.


% % \begin{figure*}[t!]
% %     \centering
% %     %\includegraphics[width=\linewidth]{figures/framework.jpg}
% %     \includegraphics[width=\linewidth]{figures/methodv2.pdf}
% %     \caption{\textcolor{orange}{The framework of our proposed two-stage retrieval method. We first retrieve the candidates through a task-agnostic retriever ($\S$\ref{sec21}), then use a task-specific prompt and pre-trained language model (PLM) to rerank the results ($\S$\ref{sec22}), finally we send the top results to the reader and give the answer ($\S$\ref{sec23}).}}
% %     \label{fig:framework}
% % \end{figure*}

% In the above tasks, question answering is typically knowledge-intensive (KI) where explicit factual knowledge can offer useful information and thus improve the results. However, besides language modeling and machine translation, it remains under-explored of the retrieval-augmented methods for Non‐Knowledge Intensive (NKI) tasks, such as sentiment analysis~\citep{10.1145/1341531.1341561cr, socher-etal-2013-recursive,pang-lee-2004-sentimental}, text classification~\citep{hovy-etal-2001-toward, li-roth-2002-learning, Wiebe2005AnnotatingEO} and linguistic acceptability~\citep{warstadt2018neural}. The challenges of leveraging retrieval-augmented method for NKI tasks are mainly two-fold:



% %Despite their impressive success on KI tasks, it remains under-explored of the retrieval-augmented methods for Non‐Knowledge Intensive (NKI) tasks, such as sentiment analysis~\citep{10.1145/1341531.1341561cr, socher-etal-2013-recursive,pang-lee-2004-sentimental}, text classification~\citep{hovy-etal-2001-toward, li-roth-2002-learning, Wiebe2005AnnotatingEO} and linguistic acceptability~\citep{warstadt2018neural}.
% % for which a large body of external knowledge and information is unnecessary
% % where the solutions to this task usually use the given training samples without retrieving explicit resources.

% %As shown in Figure \ref{fig:front}, the traditional retrievers, such as BM25~\citep{bm25} and BERT~\citep{devlin-etal-2019-bert}, can select appropriate augmented samples to help the models better understand inputs in KI tasks.
% %However, they bring negative effects on NKI tasks due to retrieving the opposite labeled samples.

% %In general, the challenges of retrieving relevant resources for NKI tasks are mainly two-fold: 
% % First, different from language modeling and machine translation tasks which focus on predicting the next token, solving NKI tasks requires overall sentence-level semantics.
% %First, \textit{relevance metrics may vary under different circumstances.} Different from KI tasks, where the goal is to introduce the required knowledge related to inputs regardless of specific tasks, the demands of retrieval to NKI tasks are diverse and task-specific. For instance, textual classification tasks need to exploit sentence-level semantics, while linguistic acceptability tasks prefer syntactic information.
% %However, existing retrievers persistently consider a single dimension of textual-level features, such as lexical overlap in BM25 and textual semantics in BERT, as shown in Figure \ref{fig:front}.
% %Therefore, since traditional retrievers are reluctant to adapt to a variety of relevance metrics for specific tasks, their retrieved results are sub-optimal in NKI tasks.
% % However, as Table~\ref{tab:intro} shows, existing retrievers such as BM25 or neural models like BERT~\cite{devlin-etal-2019-bert} and sentence-BERT~\cite{reimers-gurevych-2019-sentence} can not modeling task-specific relevance, which makes the retrieved results sub-optimal. 

% First, different from language modeling and machine translation which focus on predicting the next token, solving NKI tasks requires the overall sentence-level semantics. However, as Table 1 shows, existing sparse and dense retrievers such as BM25~\cite{bm25} and BERT~\cite{devlin-etal-2019-bert} can not model the fine-grained semantics over different tasks.

% Second, training a specific retriever for each task requires building indexes for multiple times, which can lead to high computational and memory costs. However, if we use a shared and non-trainable retriever like BM25 for all tasks, the performance could be sub-optimal due to the lack of task-specific relevance.

% %different from language model that can use the unlabeled context-token pairs, and open question answering model can leverage large-scale question-passage pairs such as in DPR (Karpukhin et al., 2020) and PAQ (Lewis et al., 2021). Training a task-specific retriever for NKI tasks is non-trivial given the limited training pairs. 

% %Also, due to the diversity of NKI tasks, to train task-specific retrievers and index the corpus for each task can lead to high computational cost.


% % language modeling that can use the unlabeled context-token pairs while 
% %Second, \textit{training retrievers for NKI tasks is non-trivial.} On the one hand, NKI tasks lack sufficient training datasets. Taking the open question answering tasks, one of the KI tasks, as an example, it can directly leverage large-scale question-passage pairs like DPR~\cite{karpukhin-etal-2020-dense} and PAQ~\cite{lewis2021paq}. 
% %However, NKI tasks are unclear in designing explicit criteria to find appropriate training pairs for supervision. 
% %On the other hand, training task-specific retrievers lead to high computational cost. Especially, building the indexes of external datastore according to different tasks is extremely resource-consuming.

% % \csj{TODO: explain the reason why we use sentence-level rather than passage-level.}
% % \textcolor{orange}{Third, \textit{it is important to choose the appropriate granularity of the external datastore.} In KI tasks, a passage-level datastore is needed as the required information about inputs always appears in a long context. However, passages can hardly help NKI tasks as they usually cannot reflect apparent task-specific features, such as sentimental tendency for sentiment analysis tasks.
% % For language modelling tasks, previous methods~\citep{khandelwal20generalization, khandelwal2021nearest} retrieve tokens for text generation, but single tokens contain too little information about the entire sentence.
% % Therefore, both passage-level and token-level external datastores are unsuitable for NKI tasks.}


% To tackle the aforementioned challenges, we propose a two-stage framework to better efficiently retrieve task-specific resources for NKI tasks. The overall framework is shown in Figure~\ref{fig:framework}. In the first stage, we use a shared dense retriever BERT to filter out most candidates in the external datastore by computing the general textual-level similarity. It is worth noting that we only build indexes once across various NKI tasks. In the second stage,  we design a series of prompts~\cite{bach2022promptsource} and leverage the auto-regressive language models~\cite{brown2020language,zhang2022opt} to further re-rank the candidates from the first stage according to the task-specific relevance similarity. Finally, we feed the nearest retrieved samples into the reader to generate answers.
% % The retrieved results are related to the training instance according to their general semantics but may not relate to the task-related attribution (\textit{e.g.}, for the sentiment analysis task, the retrieved text may not show any sentiment polarities). 

% %In the second stage, to avoid training retrievers for each task, we design a series of prompts~\cite{bach2022promptsource} and leverage the auto=regressive  language models (LLMs) to further re-rank the candidates from the first stage via task-specific relevance similarity. Finally, we feed the nearest retrieved samples into the reader model to generate answers.

% %In this way, we can not only leverage the efficiency and effectiveness advantages of traditional retrievers, but also exploit the immense potential of pre-trained models to evaluate the task-specific relevance similarity between inputs and candidates without extra training.

% % Our method can index the external resources once through the shared retriever and then re-rank the results through differently designed prompts, thus avoiding training specific retrievers and indexing the corpus for each task.
% We evaluate our method on a series of NKI tasks.
% Experimental results show that our two-stage retrieved results can stably lead to better performance compared with baselines. Our main contributions can be summarised as the following: 

% 1. To our knowledge, we are one of the few works to specifically study the retrieval-augmented methods for NKI tasks;

% 2. We propose a novel two-stage prompt-guided retrieval method to find useful resources according to task-specific relevance;

% 3. Experiments results and analysis show that our method can generally improve the performance over various NKI tasks.
